InstantStyle: Free Lunch towards Style-Preserving in Text-to-Image Generation

Tuning-free diffusion-based models have demonstrated significant potential in the realm of image personalization and customization. However, despite this notable progress, current models continue to grapple with several complex challenges in producing style-consistent image generation. Firstly, the concept of style is inherently underdetermined, encompassing a multitude of elements such as color, material, atmosphere, design, and structure, among others. Secondly, inversion-based methods are prone to style degradation, often resulting in the loss of fine-grained details. Lastly, adapter-based approaches frequently require meticulous weight tuning for each reference image to achieve a balance between style intensity and text controllability. In this paper, we commence by examining several compelling yet frequently overlooked observations. We then proceed to introduce InstantStyle, a framework designed to address these issues through the implementation of two key strategies: 1) A straightforward mechanism that decouples style and content from reference images within the feature space, predicated on the assumption that features within the same space can be either added to or subtracted from one another. 2) The injection of reference image features exclusively into style-specific blocks, thereby preventing style leaks and eschewing the need for cumbersome weight tuning, which often characterizes more parameter-heavy designs.Our work demonstrates superior visual stylization outcomes, striking an optimal balance between the intensity of style and the controllability of textual elements. Our codes will be available at https://github.com/InstantStyle/InstantStyle.

==> Sections/Ackonwledgement.tex <==
\section{Acknowledgement}
We acknowledge that there are concurrent community works\footnote{https://github.com/huggingface/diffusers/discussions/7534} that share a very similar strategy as ours, especially the selection of style blocks, however, for layout blocks (also named composition blocks in other works), we find that $4_{th}$ blocks is the most representative while other uses $3_{th}$ blocks. Another similar work is B-LoRA\cite{frenkel2024implicit}, instead of bulit on the top of IP-Adapter, they train LoRAs for specific blocks and also select $6_{th}$ blocks as style blocks. Earlier, Swapping Self-Attention\cite{jeong2024visual}  also came to a similar conclusion, but they only positioned style blocks to up blocks without a more fine-grained division. Just like infinitesimal calculus was developed independently in the late $17_{th}$ century by Isaac Newton and Gottfried Wilhelm Leibniz.
